SIMT/GPU Data Race Verification using ISCC and Intermediary Code Representations: A Case Study

It is often difficult to write code that you can ensure will be executed in the right order when programing for parallel compute tasks. Due to the way that today's parallel compute hardware, primarily Graphical Processing Units (GPUs), allows you to write code. It is easy to write code that may result in one thread reading or modifying data before it should, thus resulting in a data race. It would be useful to have a tool that could verify that the code will execute as expected. However, most static analysis done at the language level has to be completely retooled to work on a different languages. Therefore, it would be of great use to be able to perform verification and analysis on the Memory Model of a parallel compute code, in a lower level intermediary representations that most languages pass through on their way to something that the GPU hardware can understand. This body of work aims to deal with the question of if there is still enough of the information in the intermediary representations to be able to perform memory model verification to check for data races. To determine this we plan to analyze as a case study the GeSpMM Sparse Matrix Multiplication Algorithm, implemented in CUDA C++ with the LLVM compiler and Julia with CUDA.jl.

==> comm/sa-header.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% -     Package Imports       - %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{standalone}         % << Allows you to insert tables and plots from "standalone" files
\usepackage[utf8]{inputenc}     % << Required for inputting international characters.
\usepackage[T1]{fontenc}        % << Allow for better font encoding in LaTeX
\usepackage{xcolor}             % << Required to turn URLs the correct colors.
\usepackage{amsmath}            % << General math tools super useful
\usepackage{amssymb}            % << Required for using many math symbols.
\usepackage{gensymb}            % << Allow for generic symbols to be referred to by more readable names and used in both math and text modes.
\usepackage[english]{babel}     % << Allow for multi-language support in LaTeX documents
\usepackage{amsthm}             % << Allow for the use of math document sectioning (i.e. theorem, definition, etc)
\usepackage{hyperref}           % << Allow for hyper links and better reference linking and including URLs 
\usepackage{float}              % << Allow for better placement of figures tables and other position-able items.
\usepackage{wrapfig}            % << ALlow for placing figures in line with text with text wrapping
\usepackage{fancyhdr}           % << Allow for better page headers and footers
\usepackage{geometry}           % << Allow for editing page geometry
    \geometry{letterpaper}
\usepackage{changepage}         % << Allow for adjust width environment
\usepackage{mathtools}          % << required for vec projections among other things.
\usepackage{tikz, tikz-3dplot}  % << Allows for the insertion of Check-marks and drawing vector graphics
\usepackage{pgfplots}           % << Allow for the use of Graphs in document
    \usepgfplotslibrary{polar}  % << Allow for graphing of polar systems
    \pgfplotsset{compat=1.16}       % Set up compatibility mode for pgf Plots
\usepackage{subcaption}         % << Allows for the use for sub-figures to get better multi figure presentation
\usepackage{graphicx}           % << Allows you to insert images into the document, scale objects among other things
\usepackage{multicol}           % << Allows you to make tables with many columns intelligently use \begin{multicol} 
\usepackage{multirow}           % << Allows you to make tables with many rows intelligently use \begin{multirow}
\usepackage{xfrac}              % << Allows for type set slanted fractions
% \usepackage[none]{hyphenat}     % << Removes automatic hyphenation (a personal pet peeve of Sam).
\usepackage{listings,lstautogobble}     % << Allows for displaying code in a formatted way (can't be used with markdown package).
    \usepackage[mono,extrasp=0em]{inconsolata}  % <<< Allow for a better monospace font in listings and markdown code snipits
\usepackage{bm}                 % << Required to make vectors bold. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% -     Config Settings       - %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% - Font Formatting ------ 
\renewcommand{\rmdefault}{cmss}

% - listings config ----- 
\definecolor{lstIdC}{HTML}{236394}
\definecolor{lstKeyC}{HTML}{0a0a0a}
\definecolor{lstComC}{HTML}{029727}
\definecolor{lstStrC}{HTML}{F44336}

\lstset{
    float=[H],  %
    xleftmargin=1.5em,  %
    xrightmargin=.5em,  %
    breaklines, %
    breakatwhitespace=true, %
	columns=fixed,	%
    postbreak=\space,   %
    breakindent=1em,    %
    keywordstyle=\color{lstKeyC}\ttfamily\bfseries,%\small, %
    identifierstyle=\color{lstIdC}\ttfamily\bfseries,%\small,   %
    basicstyle=\ttfamily\mdseries,%\small,  %
    commentstyle=\color{lstComC}\sffamily\bfseries,%\small, %
    stringstyle=\color{lstStrC}\ttfamily\slshape,%\small,   %
    autogobble=true
    }



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% -      Notation Macros      - %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% - General Notation Macros
\newcommand{\ds}{\displaystyle}     % - used to make \displaystyle more manageable
\def\checkmark{\tikz\fill[scale=0.4](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;}    % - Creates a command to insert a check-mark symbol (requires tikz package) 

% - Better Negative Symbol
\renewcommand\neg{\,\raisebox{0.125\baselineskip}{\scalebox{1.0}[0.875]{\textbf{-}}}}	% - Used to make a proper negative sign (requires graphicx)
\newcommand\fneg{\,\scalebox{1.5}[0.875]{\textbf{-}}}									% - Used to make a proper negative sign Adjusted for fractions (requires graphicx) 

% - Vector Notations 
\newcommand{\primev}{\,\raisebox{0.125\baselineskip}{\scalebox{0.8}[0.875]{$\mathbf{'}$}}}	% - Used to make a prettier prime notation for vectors (requires graphicx)
\newcommand{\hvec}[1]{\ensuremath{\overset{\rightharpoonup}{\boldsymbol{#1}}}}  		% - Used to make a half arrow vector/harpoon notation
% \renewcommand{\vec}[1]{ \py[vh-vecNotation]{vh.vecNotation(r"#1")} }	% - Used to over-wright vec with a vec that covers all letters in it's contents (requires PythonTeX package and `vectorhelpercode.py`)
% \newcommand{\norm}[1]{\left|\!\left| #1 \right|\!\right|}    						% - Used to create a normalization annotation for vectors complex vector expressions
\newcommand{\norm}[1]{\ensuremath{\big|\!\big|#1\big|\!\big|}}    						% - Used to create a normalization annotation for vectors complex vector expressions
\newcommand{\normv}[1]{\ensuremath{\left| \vec{#1} \right|}}    					% - Used to create a normalization annotation for vectors
\newcommand{\vecf}[2][t]{\ensuremath{\vec{#2}(#1)}}                              % - Used to create a Vector Valued Function notation uses (t) by default 
\newcommand{\normvf}[2][t]{\ensuremath{\left\vert \vecf[#1]{#2} \right\vert}}     % - Used ot create a Normalized/Magnitude notation for a Vector Valued Function  

% - Vector Projection and Scalar Projection notation Commands ----
\newcommand{\vecprojnote}[3][none]{\ensuremath{\textit{Proj}_{\,\vec{#2}}\vec{#3}}} 	% - Used to make a annotation for vector projections 
\newcommand{\vecsprojnote}[3][none]{\ensuremath{\textit{Comp}_{\,\vec{#2}}\vec{#3}}}	% - Used to make a annotation for vector Scalar (Comp) projections 

% - Used to make a good sized dot to signify a dot product
\makeatletter
\newcommand*\dotp{\mathpalette\bigcdot@{.5}}
\newcommand*\bigcdot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}
\makeatother

% - Standard Vector Commands 
\newcommand{\ihat}[1]{\ensuremath{\,#1\,\boldsymbol{\Hat{i}}\,}}   % - Used to easily inert i^hat
\newcommand{\jhat}[1]{\ensuremath{\,#1\,\boldsymbol{\Hat{j}}\,}}   % - Used to easily inert j^hat
\newcommand{\khat}[1]{\ensuremath{\,#1\,\boldsymbol{\Hat{k}}\,}}   % - Used to easily inert k^hat

% - Matrix Commands
\newcommand{\mat}[1]{\ensuremath{\boldsymbol{#1}}}                       % - Create BoldFace Characters for Matrix Notation
% \renewcommand{\matrix}[1]{\ensuremath{\begin{matrix} #1 \end{matrix}]}  % - Create single line command for the Matrix Environment
\newcommand{\vecspace}[1]{\ensuremath{\boldsymbol{\mathbb{#1}}}}    % - Create notation for Vector Space Notations using mathbb font styles  


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% -        Commands           - %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand{\c}[2][]{\lstinline[#1]{#2}}      % - mask for the listings inline command for general purpose




==> tex/proposed-work/proposed-work.tex <==
% !TeX root = ..\..\main.tex

% << =========================================================================================== >> 
% <<                                      S: proposed WORK                                       >> 
% << =========================================================================================== >> 
\section{proposed Work} 

% proposed vs Proposed:
% choice: Proposed
% reason: https://oneminuteenglish.org/en/propose-or-purpose/#:~:text=When%20you%20are%20discussing%20bringing,something%2C%20you%20will%20use%20purpose.


% << =================================== Purpose Work Intro ==================================== >> 

For this project as partially described in the previous sections,
I intend to via a case study with the Ge-SpMM\cite{huang2020} algorithm
to discover if it is possible to trace the memory model of a parallel algorithm
represented in the intermediary forms of LLVM IR and CUDA PTX (ISA) in a way that 
would be meaningful to our future goal of a memory model data dependency verification tool.
%
The Ge-SpMM team has graciously provided sever implementations of its algorithm in CUDA C/C++,
with various levels of loop unrolling to increase the efficiency of the algorithm,
in their \href{https://github.com/hgyhungry/ge-spmm}{source repo}
\footnote{Ge-SpMM\cite{huang2020} source repo: 
          \href{https://github.com/hgyhungry/ge-spmm}{https://github.com/hgyhungry/ge-spmm}}.
%
I have also made an implementation of in the Julia Lang programing language\cite{bezanson2012} 
with the CUDA.jl\cite{juliagpugroup2021} 
library that enables CUDA programing in Julia.
%
For C/C++ implementations we will compile to LLVM IR and PTX using the Clang compiler.
%
Additionally, since Julia is a Just in Time (JiT) programing language implemented with LLVM
and the CUDA.jl package \cite{juliagpugroup2021} operates such that it just uses same LLVM 
provided CUDA compilation pathway 
after scrubbing away some of the unessisary Julia components from the LLVM IR representation
to get the kernel code, we can also get the requisite LLVM IR and PTX representations
from our Julia code as well,
but with some extra Julia information in at least the LLVM IR if not also the PTX representations.


This extra information, from Julia that possibly exists in the intermediary representations,
is one of the biggest reasons we chose to look at CUDA kernels compiled from Julia to begin with.
%
As comparing it to any code from the much more low-level CUDA-C/C++ algorithms will help us 
differentiate extra information that higher level languages might leave in their intermediary representations durning compilations.
%
%? NOTE: this thought is still ill-formed in my head.
% Additionally, Julia is a popular language for scientists and mathematicians to crunch numbers with,
% and as is common in such languages arrays start with 1,
% complicating 


From this state I will determine if there components I need can be located or at least derived 
from the intermediary code representations.
%
Those components being:
(1) function/kernel header information, especially as it has to do with input and output data parameters;
(2) basic typing information for arrays, pointers, floats and the various integral types;
(3) kernel/driver calls to retrieve thread, block and tile coordinate information;
(4) kernel/driver calls to any of the built in thread fencing ``functions;''
(5) kernel/driver calls to retrieve a memory location for a section of shared memory;
(6) pointers to memory locations inside any array;
and finally (7) when/where data is being combined and moved around.
%
To do it, first we will need to identify calls to any driver functions and reserved registers,
make sure we can identify what call and/or information it relates too.
%
Then we will attempt a manual data trace of the elements of the data to better our understanding,
before using whatever integer set tool we find most useful.
%
Be that tool the iscc interactive calculator\cite{verdoolaege2013}, 
directly using the Integer Set Library (ISL) \cite{kruse2021a} that iscc uses,
or possibly using the Alloy tool\cite{jackson1997}.
%
If the Alloy tool can be adapted to the work,
since it is a set based verification tool that we are familiar with
and is far more fully fledged in terms of visualizations and human intractable 
components than many of these domain specific tools.
%
This would be useful given how manual and human focused this body of work's tasks are,
but is not nearly as easily adaptable to use with our future work.


If all goes well, and it seems possible that there is a way to identify all the elements we need 
to perform our analysis, and we have time we may move on to analyzing at least one known bad algorithm in
a similar manner
to see if it affects our ability to work with the intermediary representations.
%
But in the end we hope to have been able to better our understanding of the mechanics of parallel algorithms
and the effects of various forms code representations has on the information that can be derived
from said representations
in terms of what we need to perform our future memory model analysis on data-dependencies and data-races,
in our planned future work.



% << =========================================================================================== >> 
% <<                                     SUBSECTION INCLUDES                                     >> 
% << =========================================================================================== >> 

\newpage
%- ss - Schedule ----------- 
% \input{tex/proposed-work/schedule}  % not necessary in my thesis.


%? END section {proposed Work}

==> tex/proposed-work/schedule.tex <==
% !TeX root = ..\..\main.tex

% << =========================================================================================== >> 
% <<                                         S: SCHEDULE                                         >> 
% << =========================================================================================== >> 
\subsection{Schedule}


 % << ===================================== Schedule Intro ====================================== >> 

 \begin{table}[H]
  \centering
  \begin{tabular}{cc|l|}
  \hline
      
                  [\checkmark] & \textit{est.} Compl. Date\footnotemark[5]
               & 
                  Task description
               \\ \hline
      
                  [\checkmark] & 06/01
               & 
                  Learn CUDA C/C++ and generic GPU Programing (for CUDA)
               \\
      
                  [\checkmark] & 06/07
               & 
                  Learn about the memory model issues in parallel programing
                  
               \\
      
                  [\checkmark] & 06/15
               & 
                  Learn about memory optimization patterns in CUDA GPUs
               \\
      
                  [\checkmark] & 07/24
               & 
                  Learn Julia\cite{bezanson2012} and CUDA.jl\cite{juliagpugroup2021}
               \\
      
                   [\checkmark] & 09/20
               & 
                  Implementing a generic
                          Ge-SpMM\cite{huang2020} implementation in Julia \footnotemark[6]
               \\
      
                   [\checkmark] & 10/04
               & 
                  Learn LLVM IR and CUDA PTX (ISA) to a workable degree (Possibly some SASS too)
               \\
      
                  [~ ~] & ??/??\footnotemark[7]
               & 
                  Eval paths from Julia $\rightarrow$ LLVM $\rightarrow$ CUDA/PTX (CUDA.jl vs in-house beta
                          AST)\footnotemark[8]
               \\
      
                   [\checkmark] & 10/20
               & 
                  Identify the components in the Intermediary syntaxes important to our planned verification process
               \\
      
                   [\checkmark] & 11/01
               & 
                  Design standardized test/experiment procedures for the case study
               \\
      
                   [~ ~] & 11/15
               & 
                  Perform case study on the various algorithms to discover if req elm
                          are present.
               \\
      
                   [~ ~] & 11/29
               & 
                  Analyze data and draw conclusion for thesis
               \\
  \end{tabular}
  \label{tab:schedule}
  \caption{Rough schedule and plan of tasks to complete for the research.}
\end{table}
\footnotetext[5]{some dates may no longer be accurate for currently incomplete tasks, as the usual craziness of end of semester projects has severally slowed down work on this project.}
\footnotetext[6]{CUDA C++ code provided by the GeSpMM team\cite{huang2020} at \href{https://github.com/hgyhungry/ge-spmm}{https://github.com/hgyhungry/ge-spmm}}
\footnotetext[7]{Not entirely sure if we will do this task at all, and therefore at what time we would require it to be done.}
\footnotetext[8]{Tanmay Tirpankar, a fellow researcher, has been working on an approach for analyzing Julia code via a custom AST interpretation in the LLVM ecosystem that we might end up using.}




%? END subsection {Schedule}

==> tex/results/case-study.tex <==
% !TeX root = ..\..\main.tex

% << =========================================================================================== >> 
% <<                                  SS: PTX ANALYSIS RESULTS                                   >> 
% << =========================================================================================== >> 
\subsection{Results of the Case Study on Ge-SpMM}\label{sec:ge-spmm-results}

... Filler text ...



%? END tex/results/ptx.tex

==> tex/results/our-methods.tex <==
% !TeX root = ..\..\main.tex

% << =========================================================================================== >> 
% <<                                SS: LLVM-IR ANALYSIS RESULTS                                 >> 
% << =========================================================================================== >> 
\subsection{}

... Filler text ...



%? END tex/results/ptx.tex
